To vote, or not to vote: on the epidemiological impact of electoral campaigns at the time of COVID-19

Elections are crucial for legitimating modern democracies, and giving all candidates the possibility to run a proper electoral campaign is necessary for elections' success in providing such legitimization. Yet, during a pandemic, the risk that electoral campaigns would enhance the spread of the disease exists and is substantive. In this work, we estimate the causal impact of electoral campaigns on the spread of COVID-19. Exploiting plausibly exogenous variation in the schedule of local elections across Italy, we show that the electoral campaign preceding this latter led to a significant worsening of the epidemiological situation related to the disease. Our results strongly highlight the importance of undertaking stringent measures along the entire electoral process to minimize its epidemiological consequences.

==> table_results_region_controls.tex <==
\begin{tabular}{lcccccc} \hline\hline
  & (1) & (2) & (3) & (4) &(5) & (6)   \\
& Infections & Tests &  \% Posit  & Hospit.  &  ICUs & Deaths  \\ 
 \hline
 &  &  &  & &  &   \\
 Campaign $\times$ Post & 0.070*&-0.083***&0.420*&0.240***&0.053**&0.006* \\
 & (0.033)&(0.019)&(0.18)&(0.052)&(0.020)&(0.002)\\
 &  &  &  &   &  &    \\
Observations &2,060&2,060&2,060&2,060&2,060&2,060\\
Mean Dep. Var. &0.602&4.437&1.208&0.851&0.119&0.014\\
Region  FE &\checkmark&\checkmark&\checkmark&\checkmark &\checkmark&\checkmark  \\
Pre-trends in observables & \checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark \\
 Date $\times$ Adjacent reg. FE &\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark\\
 \hline\hline
\end{tabular}


==> table_weight_regional_boundary.tex <==
\begin{tabular}{lcccccc} \hline\hline
  & (1) & (2) & (3) & (4) &(5) & (6)   \\
& Infections & Tests &  \% Posit.  & Hospit.  &  ICUs & Deaths  \\ 
 \hline
 &  &  &  & &  &   \\
 Campaign $\times$ Post & 0.070*&-0.083***&0.146***&0.240***&0.053**&0.006* \\
 & (0.033)&(0.019)&(0.031)&(0.052)&(0.020)&(0.002)\\
 &  &  &  &   &  &    \\
Observations &2,060&2,060&2,060&2,060&2,060&2,060\\
Baseline (value) &0.315&83.578&0.404&0.904&0.0032&0.012\\
Region  FE &\checkmark&\checkmark&\checkmark&\checkmark &\checkmark&\checkmark  \\
Regional pre-trends & \checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark \\
 Date $\times$ Adjacent reg. FE &\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark\\
 \hline\hline
\end{tabular}

